Test-Time Adaptation for Speech Emotion Recognition

The practical utility of Speech Emotion Recognition (SER) systems is undermined by their fragility to domain shifts, such as speaker variability, the distinction between acted and naturalistic emotions, and cross-corpus variations. While domain adaptation and fine-tuning are widely studied, they require either source data or labelled target data, which are often unavailable or raise privacy concerns in SER. Test-time adaptation (TTA) bridges this gap by adapting models at inference using only unlabeled target data. Yet, having been predominantly designed for image classification and speech recognition, the efficacy of TTA for mitigating the unique domain shifts in SER has not been investigated. In this paper, we present the first systematic evaluation and comparison covering 11 TTA methods across three representative SER tasks. The results indicate that backpropagation-free TTA methods are the most promising. Conversely, entropy minimization and pseudo-labeling generally fail, as their core assumption of a single, confident ground-truth label is incompatible with the inherent ambiguity of emotional expression. Further, no single method universally excels, and its effectiveness is highly dependent on the distributional shifts and tasks.

==> Sections/02-relatedwork.tex <==
\section{Related Work}
Transfer learning is one of the most commonly used adaptation methods for adapting SER~\cite{marczewski2017learning}, but it requires a substantial amount of labeled data from the target domain, while emotion annotation is label-intensive. A recent study explored parameter-efficient fine-tuning methods for adaptation from acted to natural emotion speech and demonstrated effectiveness. However, this approach still requires labeled speech data~\cite{lashkarashvili2024parameter}.
Additionally, unsupervised domain adaptation, which requires only a small amount of target domain speech data without labels, has been proposed~\cite{xu2024kwformer, zhao2024layer}. These methods aim to learn domain-invariant feature representations by using both source and target domain data simultaneously during the training process. However, accessing target domain data is not always feasible, especially in the health domain, where privacy is a concern, and in unpredictable real-world scenarios with new, unseen data.

\td{to continue}Test time adatpation, which adapts the models during the run time without 
